ASL-Skeleton3D and ASL-Phono: Two Novel Datasets for the American Sign Language

Sign language is an essential resource enabling access to communication and proper socioemotional development for individuals suffering from disabling hearing loss. As this population is expected to reach 700 million by 2050, the importance of the language becomes even more essential as it plays a critical role to ensure the inclusion of such individuals in society. The Sign Language Recognition field aims to bridge the gap between users and non-users of sign languages. However, the scarcity in quantity and quality of datasets is one of the main challenges limiting the exploration of novel approaches that could lead to significant advancements in this research area. Thus, this paper contributes by introducing two new datasets for the American Sign Language: the first is composed of the three-dimensional representation of the signers and, the second, by an unprecedented linguistics-based representation containing a set of phonological attributes of the signs.

==> en/abstract_structured.tex <==
\textit{Background:} Sign language is an essential resource enabling access to communication and proper socioemotional development for individuals suffering from disabling hearing loss, whose population is expected to reach 700 million by 2050. Sign Language Recognition (SLR), in turn, aims to bridge the gap between users and non-users of such language. However, the scarcity in quantity and quality of sign language datasets is one of the main challenges limiting the exploration of novel approaches that could lead to significant advancements in the SLR. 

\textit{Method:} This paper introduces two datasets derived from the American Sign Language Lexicon Video Dataset (ASLLVD). The first one is composed of the 3D coordinates of the signers, computed from multiple images of the original sign's articulation. The second includes an unprecedented linguistics-based representation, consisting of phonological attributes computed from the 3D space described by the coordinates above.

\textit{Conclusion:} The two datasets are essential assets to contribute to the SLR field because, while addressing the challenge above, they enable researchers 1) to derive new representations such as embeddings or new datasets from the 3D coordinates and 2) to explore new techniques based on the sign language linguistics, which is a common starting point for humans when learning and understanding languages.
